Local Structure Matters Most: Perturbation Study in NLU

Recent research analyzing the sensitivity of natural language understanding models to word-order perturbations has shown that neural models are surprisingly insensitive to the order of words. In this paper, we investigate this phenomenon by developing order-altering perturbations on the order of words, subwords, and characters to analyze their effect on neural models' performance on language understanding tasks. We experiment with measuring the impact of perturbations to the local neighborhood of characters and global position of characters in the perturbed texts and observe that perturbation functions found in prior literature only affect the global ordering while the local ordering remains relatively unperturbed. We empirically show that neural models, invariant of their inductive biases, pretraining scheme, or the choice of tokenization, mostly rely on the local structure of text to build understanding and make limited use of the global structure.

==> Reproducibility_Checklist.tex <==
\twocolumn
\section{Reproducibility Checklist}
\label{app:reproducibility}
As per the prescribed Reproducibility Checklist, we provide the information of the following:

\begin{itemize}
    \item \textit{A clear description of the mathematical setting, algorithm and/or model}: We provide details of models used in \S\ref{sec:experiments-main} and \S\ref{app:pseudocode_perturbations} for
     detailing pseudocodes for both the metrics and the different perturbations proposed in the paper.
    \item \textit{Submission of source code}: Source code for the perturbations, metrics and models is provided in \href{https://github.com/chandar-lab/SyntaxStudy}{GitHub}.
    The training code was adapted from the excellent \citet{HuggingFace} github.
    \item \textit{Description of the computing infrastructure used}: We used up to 20 NVIDIA V100 32 GB at a time to run all experiments. All models where trained and evaluated on 1 NVIDIA V100 32 GB GPUs for every seed of every model. 
    \item \textit{Average runtime for each approach}: The approximate training time for fine-tuning varies between $4$-$8$ hours and the inferencing on standard validation sets was about an hour.
    \item \textit{Explanation of evaluation metrics used, with links to code}: We add necessary citations for the metrics considered in the paper and also provide codes to reproduce them.
    \item \textit{Relevant statistics of the datasets used}: We provide the statistics of the datasets used in \ref{sec:experiments-main}.
    \item \textit{Explanation of any data that were excluded, and all pre-processing steps}: The details for omitting WNLI data from GLUE benchmark are provided in \S\ref{app:experiments}. 
    \item \textit{Link to downloadable version of data}: The data sets used in the paper are from public repositories. Links to the paper that proposes the data sets is included in \S\ref{sec:experiments-main}.
\end{itemize}

==> listings.tex <==
\begin{lstlisting}[float=ht!,breaklines=true,caption={
Python style pseudocode to calculate the IDC metric.},language=Python]
# Perturbed list of indexes of the original characters position
X_p      
# List of absolute distance to original positions
IDC_list = []       

for i in range(len(X_p)):
    absolute_distance_to_original_position = abs(i - X_p[i])
    IDC_list.append(absolute_distance_to_original_position)

# Average absolute distance to original position
IDC_agg = mean(IDC_list) 

# Normalization by the length of the text
IDC = IDC_agg / len(X_p) 
\end{lstlisting}


\begin{lstlisting}[float=ht!,breaklines=true,caption={
Python style pseudocode to calculate the DND metric.},language=Python]
# Perturbed list of indexes of the original characters position
X_p           
# List of broken neighbouring relationships
DND_list = [] 

for i in range(len(X_p) - 1):

    # If the following character is the next one in the original order
    if X_p[i] - X_p[i + 1] == 1: 
        DND_list.append(0)
    else:
        DND_list.append(1)

# Sum the amount of broken neighbour
DND_agg = sum(DND_list)       

# Normalization by the total amount of neighbour
DND = DND_agg / (len(X_p) - 1) 
\end{lstlisting}


\begin{lstlisting}[float=ht!,basicstyle=\ttfamily\scriptsize,breaklines=true,caption={
A few example of perturbations as well as the calculation steps to obtain both the IDC and DND metrics.}]
# Original order
X           = "T  h  i  s ' ' i  s ' ' a ' ' t   e   s   t"
P_X         = [0, 1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13]

# Simple splitting along the middle 
X'          = "a ' ' t   e   s   t   T  h  i  s ' ' i  s ' '"  
P_X'        = [8, 9, 10, 11, 12, 13, 0, 1, 2, 3, 4, 5, 6, 7] 

IDC_list    = [8, 8, 8,  8,  8,  8,  6, 6, 6, 6, 6, 6, 6, 6]
IDC_agg     = 6.85
IDC         = 0.49 

DND_List    = [0, 0, 0,  0,  0,  0,  1, 0, 0, 0, 0, 0, 0] 
DND_agg     = 1   
DND         = 0.08            

# Shuffling of the words randomly
X'          = "t   e   s   t   i  s ' ' a ' ' T  h  i  s ' '" 
P_X'        = [10, 11, 12, 13, 5, 6, 7, 8, 9, 0, 1, 2, 3, 4] 

IDC_list    = [10, 10, 10, 10, 1, 1, 1, 1, 1, 9, 9, 9, 9, 9]   
IDC_agg     = 6.42                          
IDC         = 0.46                

DND_List    = [0,  0,  0,  1,  0, 0, 0, 0, 1, 0, 0, 0, 0]   
DND_agg     = 2                             
DND         = 0.15           

# Flipping neighbouring characters randomly
X'          = "h  T  i ' ' i  s ' ' s  a ' ' t   s   e   t" 
P_X'        = [1, 0, 2, 4, 5, 3, 7, 6, 8, 9, 10, 12, 11, 13]

IDC_list    = [1, 1, 0, 1, 1, 2, 1, 1, 0, 0, 0,  1,  1,  0]
IDC_agg     = 0.71     
IDC         = 0.05                 

DND_List    = [1, 1, 1, 0, 1, 1, 1, 1, 0, 0, 1,  1,  1]
DND_Agg     = 10  
DND         = 0.76        



\end{lstlisting}

\newpage
%\onecolumn
\section{Perturbations Pseudocode}\label{app:pseudocode_perturbations}

\begin{lstlisting}[float=ht!,breaklines=true,caption={
Python style pseudocode to performing a phrase shuffle.},language=Python]
# Probability of a token being the last of the current phrase
rho = 0.5                
# Text to be shuffled, split on the chosen granularity
text                    
all_phrases = []
phrase = [text[0]]

# Iterate through the text on the chosen granularity
for token in text[1:]:  

    # Uniform distribution between 0 and 1
    prob = random()     
    if prob < rho:
        all_phrases.append(phrase)
        phrase = [token]
    else:
        phrase.append(token)

all_phrases.append(phrase)    
phrase_shuffled_text = ''.join(shuffle(all_phrases))

\end{lstlisting}


\begin{lstlisting}[float=ht!,breaklines=true,caption={
Python style pseudocode to performing a neighbour flip shuffle.},language=Python]

# Probability of a token being flipped with the next token
rho = 0.5              
# Text to be shuffled, split on the chosen granularity
text                    

perturbed_tokens = []
held_token = text[0]

# Iterate through the text on the chosen granularity
for token in text[1:]:  

    # Uniform distribution between 0 and 1
    prob = random()     
    if prob < rho:
        perturbed_tokens.append(held_token)
        held_token = token 
    else:
        perturbed_tokens.append(token)
perturbed_tokens.append(held_token)    

neighbour_flip_shuffled_text = ''.join(perturbed_tokens)

\end{lstlisting}
